360 in the Wild: Dataset for Depth Prediction and View Synthesis

The large abundance of perspective camera datasets facilitated the emergence of novel learning-based strategies for various tasks, such as camera localization, single image depth estimation, or view synthesis. However, panoramic or omnidirectional image datasets, including essential information, such as pose and depth, are mostly made with synthetic scenes. In this work, we introduce a large scale 360$^{\circ}$ videos dataset in the wild. This dataset has been carefully scraped from the Internet and has been captured from various locations worldwide. Hence, this dataset exhibits very diversified environments (e.g., indoor and outdoor) and contexts (e.g., with and without moving objects). Each of the 25K images constituting our dataset is provided with its respective camera's pose and depth map. We illustrate the relevance of our dataset for two main tasks, namely, single image depth estimation and view synthesis.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


***************************** Subdirectories ******************************

bibtex   - The IEEEtran BibTeX style package.

extras   - Supplementary material that may be of interest.

testflow - The testflow diagnostic suite for verifying PS/PDF output.

tools    - The IEEEtrantools.sty package which provides several commands
           from the IEEEtran.cls file for use with other LaTeX classes.


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex,
                   bare_jrnl.tex, bare_jrnl_comsoc.tex,
                   bare_jrnl_compsoc.tex, bare_jrnl_transmag.tex
***************************************************************************


==> figures/figure.tex <==
\begin{table*}
\renewcommand{\arraystretch}{1.15}
\resizebox{\textwidth}{!}{
\centering

\begin{tabular}{cccc ccccc ccc}

% 92tbuDu72QY-2 - mannequin-1
% 9XR2CZi3V5k-2 - outdoor-1
% gwDTx5m5Elk-3 - indoor-1


% JeA6jyhHEbc_room2 - Mannequin-2 
% I1sUO5mnT6k_room1 indoor mask-1(m1)
% bN5OEyV_uQ0_room3 indoor mask-2


\multirow{2}{*}{ } & \multicolumn{4}{c}{\bfseries Mannequin-1} & \multicolumn{4}{c}{\bfseries Outdoor-1} & \multicolumn{3}{c}{\bfseries Indoor-1} \\ \cline{2-4}  \cline{6-8} \cline{10-12}
                        & $\uparrow$PSNR & $\uparrow$SSIM & $\downarrow$LPIPS & 
                        & $\uparrow$PSNR & $\uparrow$SSIM & $\downarrow$LPIPS &
                        & $\uparrow$PSNR & $\uparrow$SSIM & $\downarrow$LPIPS \\

NeRF++~\cite{nerfpp} & 17.68             & 0.510             & 0.657                 &       & 25.83             & 0.721             & 0.443             &            & \bfseries 19.37  & 0.656             & 0.500\\
Ours                 & \bfseries 19.14   & \bfseries 0.610   & \bfseries 0.267       &       & \bfseries 26.57   & \bfseries 0.763   & \bfseries 0.269   &           & 18.75            & \bfseries 0.663   & \bfseries 0.330 \\
\hline

\multirow{2}{*}{ } & \multicolumn{4}{c}{\bfseries Mannequin-2} & \multicolumn{4}{c}{\bfseries Indoor-m1} & \multicolumn{3}{c}{\bfseries Indoor-m2} \\ \cline{2-4}  \cline{6-8} \cline{10-12}
                        & $\uparrow$PSNR & $\uparrow$SSIM & $\downarrow$LPIPS & 
                        & $\uparrow$PSNR & $\uparrow$SSIM & $\downarrow$LPIPS &
                        & $\uparrow$PSNR & $\uparrow$SSIM & $\downarrow$LPIPS \\

NeRF++~\cite{nerfpp} & 14.38             & 0.344             & 0.637                 &       & 14.60             & 0.403             & 0.649             &            &  13.00                  & 0.423             & 0.690\\
Ours                 & \bfseries 16.72   & \bfseries 0.539   & \bfseries 0.429       &       & \bfseries 15.88   & \bfseries 0.497   & \bfseries 0.442   &           & \bfseries14.46            & \bfseries 0.564   & \bfseries 0.421 \\
\hline

\end{tabular}
}\label{tbl:nerfpp_and_ours}
\caption{\textbf{Quantitative view synthesis results on the 360$^\circ$ in the wild}. Experiment on various environments including the 3 categories and masked input sequence with masked region on moving object~(\eg capturing person). Note that we experiment multi-scale structural similarity for SSIM. Our result outperforms across every metrics by significant difference. } %\label{table:nerfpp_and_ours}
\end{table*}

==> figures/table_result_synthesis.tex <==
\begin{table*}
\renewcommand{\arraystretch}{1.5}
\centering
\resizebox{0.9\textwidth}{!}{
\begin{tabular}{c ccc ccccc ccc}

% 92tbuDu72QY-2 - mannequin-1
% 9XR2CZi3V5k-2 - outdoor-1
% gwDTx5m5Elk-3 - indoor-1
% JeA6jyhHEbc_room2 - Mannequin-2 
% I1sUO5mnT6k_room1 indoor mask-1(m1)
% bN5OEyV_uQ0_room3 indoor mask-2
\hline
\multirow{2}{*}{ } & \multicolumn{4}{c}{ Mannequin-1} & \multicolumn{4}{c}{ Outdoor-1} & \multicolumn{3}{c}{ Indoor-1} \\ \cline{2-4}  \cline{6-8} \cline{10-12}
                        & $\uparrow$PSNR & $\uparrow$SSIM & $\downarrow$LPIPS & 
                        & $\uparrow$PSNR & $\uparrow$SSIM & $\downarrow$LPIPS &
                        & $\uparrow$PSNR & $\uparrow$SSIM & $\downarrow$LPIPS \\

%Vanilla NeRF++~\cite{nerfpp} & 17.68             & 0.510             & 0.657                 &       & 25.83             & 0.721             & 0.443             &            &  \bfseries 19.37  & 0.656             & 0.500\\
Extended NeRF++                 &  19.14   &  0.610   &  0.267       &       &  26.57   &  0.763   &  0.269   &           & 18.75            &  0.663   &  0.330 \\
\hline

\multirow{2}{*}{ } & \multicolumn{4}{c}{ Mannequin-2} & \multicolumn{4}{c}{ Indoor-m1} & \multicolumn{3}{c}{ Indoor-m2} \\ \cline{2-4}  \cline{6-8} \cline{10-12}
                        & $\uparrow$PSNR & $\uparrow$SSIM & $\downarrow$LPIPS & 
                        & $\uparrow$PSNR & $\uparrow$SSIM & $\downarrow$LPIPS &
                        & $\uparrow$PSNR & $\uparrow$SSIM & $\downarrow$LPIPS \\

%Vanilla NeRF++~\cite{nerfpp} & 14.38             & 0.344             & 0.637                 &       & 14.60             & 0.403             & 0.649             &            &  13.00                  & 0.423             & 0.690\\
Extended NeRF++                 &  16.72   &  0.539   &  0.429       &       &  15.88   &  0.497   &  0.442   &           & 14.46            &  0.564   &  0.421 \\
\hline

\end{tabular}
}
\vspace{2.3mm}
\caption{Quantitative analysis of the 360$^\circ$ view synthesis from our NeRF++ for panormaic views. We test various environments, including images with masked regions of moving objects~(\eg, capturing person). We evaluate the results with PSNR, multi-scale structural similarity for SSIM~\cite{wang2004image}, LPIPS~\cite{zhang2018unreasonable}. \FR{we need an analysis in the text about these results .. but since we do not have comparison now it is very empty // also I need to rethink the table entirely ...}
%In most cases, our extended NeRF++ outperforms across every metric by a significant difference. The examples of the results are shown in \Fig{qual_nerfpp_and_ours} and \Fig{mask_remove}. /FR{Please, Need to discuss about this table. If we remove the Vanilla Nerf, the table will look a bit empty. Is it okay to you? I will modify as soon as you give me your opinion}
}
\label{tbl:nerfpp_and_ours}
\end{table*}

==> misc/BackupLongText.tex <==
\iffalse
\FR{For decades, estimating the 3D structure of the scene required multiple images acquired from different viewpoints. Recently, machine learning based strategies allowed to take advantage of monocular cues to perform single image depth estimation. One of the earliest approach was proposed by Eigen~\etal~\cite{eigen2014depth}. In this seminal work, a coarse-to-fine strategy is presented to regress a dense depth map from a single input view . Despite various limitations regarding the quality and the resolution of the resulting depth map, this pioneering work paved the way toward more accurate techniques. In particular, the development of ordinal depth estimation further improved the quality of the scene reconstruction from a single view [XX]. While previously mentioned methods provide an accurate estimate of the depth, their training process requires a supervision from a large set of ground-truth depth maps. To reduce this data dependence, multiple self-supervised strategies have been proposed [XX]. Specifically, these approaches learn depth prediction from video sequences such that the training signal can be provided via photo-consistency constraints across successive views. These approaches have been designed for perspective cameras only and are not adequate for images containing strong geometric distortions and non-linear resolution. 
To deal with these limitations, novel methods have been developed specifically for panoramic images. 
In this regard, OmniDepth~\cite{omnidepth} was one of the first work to address single image equirectangular depth reconstruction. Omnidepth proposes a large set of synthetic $360^{\circ}$ images and their corresponding ground-truth depth maps.\kb{Omnidepth was extended to~\cite{zioulis2019spherical} which present self-supervised learning in stereo system. }
As an alternative, to alleviate the limited quantity of $360^{\circ}$ depth annotated images, Payen et al.~\cite{payen2018eliminating} approached depth estimation as a domain adaptation problem between labelled perspective and unlabeled omnidirectional data. 
More recently, novel network architectures specifically designed for omnidirectional images have been developed. It is for instance the case of BiFuse~\cite{bifuse} where a bi-projection fusion takes advantage of two different representations (namely the cube map and the equirectangular images). While this strategy led to significant improvements, it relies on a rather complex set of networks. As an alternative, \cite{chen2020distortion} address the limitations of conventional convolution via a deformable convolution which is more appropriate to equirectangular images.}
\FR{In the context of single image depth estimation, our dataset is particularly pertinent. Specifically, it can be used for multiple purposes, such as, single image depth training and self-supervised depth estimation (thanks to the sequential nature of our data). Moreover, it is a useful benchmark to evaluate depth estimation in the context of $360^\circ$ images. }
%Among these works, we experimented with~\cite{bifuse,omnidepth} which codes are released publicly.
\kb{Among these works, we experimented with~\cite{zioulis2019spherical} which consist of both supervised learning with single image and self-supervised learning with stereo/trinocular camera set-up. \cite{zioulis2019spherical} have potential to expand the proposed model's capacity to estimate the depth in monocular video sequence, predicting successive camera pose which is not studied now. Therefore, in experimental section, we show the benchmark results for the expand-ability of~\cite{omnidepth,zioulis2019spherical}. }
\fi


\iffalse
\FR{To synthesize novel images from various viewpoints, NeRF~\cite{nerf} proposes to represent a 3D scene as a neural radiance field. Concretely, this representation is learned by a network which maps a 5D vector ($(x,y,z)$ location of a 3D point and its viewing direction~$(\theta,\phi)$) to RGB color values and opacity (4D vector). This mapping can be used to render novel views using conventional volume rendering methods. }
\FR{Given a set of $N$ training images (static scene) alongside with their respective poses, NeRF approximates the continuous 5D scene representation using a fully-connected neural network $F_{\Theta} : (x,y,z,\theta,\phi) \rightarrow (r,g,b,\sigma)$, where $\Theta$ stands for the network's parameters to be optimized. For convenience, we will use $\mathbf{c}$ and $\mathbf{d}$ to expressed the color and the viewing direction vector respectively. Since the volume rendering is fully differentiable, the network can learn the radiance field representation of the scene by minimizing the photometric error $\mathcal{L}$ between the $i^{th}$ original image $I_i$ and its corresponding rendered image $\hat{I}_i$ as follows:
\begin{equation}
    \mathcal{L} = \min_{\sigma, \mathbf{c}} \frac{1}{n} \sum_{i=1}^{N} 
    \norm{ (I_i - \hat{I}_i(\sigma, \mathbf{c}))}^2_2.
\end{equation}
To perform the volume rendering, a 1D integral along each pixel's ray have to be performed. This integration is approximated in a discrete manner via a sampling strategy along each ray. First, a coarse normal sampling is used to establish a probability distribution from which a second (finer) sampling is performed around the object's boundaries.
While this hierarchical sampling allows to drastically reduce the needed number of samples, it requires to empirically set a lower and an upper bounds in which the points are selected. This bounded volume representation becomes problematic when the objects are located outside of this range or when the scene is very large (under sampling condition). This phenomenon has been recently highlighted in NeRF++~\cite{nerfpp}. When the dynamic range of the true scene depth is large, the original sampling strategy proposed in~\cite{nerf} can hardly describe the volume, leading to inaccurate and blurry image synthesis. To cope with this issue, NeRF++ proposes a new formulation for unbounded scenes. This new parametrization is called \emph{inverted sphere parameterization}. First of all, the largest distance between the cameras' centers is used to rescale the translations. Thus, the representation is partitioned in two distinct volumes: the inner (foreground) and the outer (background) volumes. These two volumes are approximated via two separated NeRFs. The foreground points lie in the inner volume defined by a sphere of unit radius in which the sampling is performed similarly to the vanilla NeRF. On the contrary, the points in the outer volume are sampled in an unbounded fashion $[0, \infty]$. To sample 3D points in this volume (when $\sqrt(x^2 + y^2 + z^2)>1$) an homogeneous coordinate representation is proposed $(x',y',z',1/r)$, where $(x',y',z')$ is a unit vector along $(x,y,z)$ and $r$ is a value from which we sample in a range $[0,1]$. When $r$ tends to zero, the sampled points are near infinity while a larger $r$ sample points closer to the inner volume. Finally, the volume rendering integral can be rewritten as the summation of the integrals from both the inner and the outer volume.
}

\FR{NeRF and its follow-up NeRF++ achieves compelling performances but have not been specifically designed for spherical cameras which reduce their applicability to perspective sensors. In this paper, we propose to adapt such approaches for the particular case of panoramic images. Two major components have to be considered. First of all, the pixel rays have be computed accordingly with the specific geometry of $360^\circ$ images. Second, the bounds of the reconstruction volume have to be adjusted such that the entire scene can be taken into consideration.
For a full panoramic image, the computation of the camera's rays is trivial and does not require any calibration parameters. Given a panorama $P$ of size $H \times W$, each pixel $(p_x,p_y) \in P$ can be expressed into spherical coordinates $(p_\theta,p_\phi)$. This conversion is performed via a linear mapping $p_\theta\in(0,2\pi)$ and $p_\phi \in (-\pi/2, \pi/2)$. Finally, the rays' direction is expressed in Euclidean coordinates on the Gaussian sphere which can be directly used in the NeRF and NeRF++ pipelines.
The original NeRF implementation considers a bounded cost volume located in front of a reference camera. While this assumption is valid for perspective cameras, it is not compatible for omnidirectional vision systems. A plausible solution would be to center the volume at the cameras' mean position. However, far away objects (located outside of this volume) would be badly reconstructed. Thus, we privileged the dual volumes strategy proposed by NeRF++ since it explicitly considers the entire surrounding scene by its spherical nature and it also accounts for the far away objects via an unbounded sampling technique.
In this paper, we selected our modified version of NeRF++ as a baseline for multiple reasons. First NeRF (and its variants) are currently state-of-the-art in view synthesis. Moreover, its simple structure can be easily adapted to spherical cameras without any approximation. Finally, we decided to use NeRF++ instead of NeRF for more flexibility since our dataset contains various types of scenes with far and near-by objects.}


\FR{While perspective image datasets providing accurate camera pose are abundant [XX,XX,XX], it is not the case for panoramic images. Thus, this dataset constitutes a solid benchmark for the development and testing of view synthesis techniques. Moreover, the variety of our data contains relevant challenges for view synthesis, such as large environments and complex indoor scenes. Finally, the large number of ``frozen people" in the dataset makes it applicable to scene containing moving persons. }

\fi

\iffalse
NeRF++~\cite{nerfpp} proposed a new geometrical representation called inverted sphere parameterization to deal with this problem. 
 In nerf++, a new sphere representation was built to compensate for this problem. After normalization of converting the maximum distances with all cameras to 1, the world coordinate center is set as the avg camera center. (ray vector expressed in the world coordinate)
 
 However, when the depth is sampled in inside the circle, it can be derive as in eq 1., but in the case of a point outside the circle, w is calculated from sampled depth(r) and the ray is expressed as 1/r, so that convergence of integral sum is guaranteed.
 
However, We do further and extended this expression into 360. 
Each camera ray expressed as perpective was transformed to referential 360 camera, indicating a spherical ray (showing the equation). 

And to see the difference between nerf and nerf++, an experiment was conducted in the experimental section. \kb{todo: do some exp nerf and nerf++ with spherical ray}
Interestingly, if you use 360 video, ~ (maybe it will converge better because scenes overlap often and there is no outward limit?)
in center camera and input camera
\fi

\iffalse
The spread of compact and smart devices with a camera enables people to create diverse video content anytime. 
%Various real-world videos are converted and processed for omnidirectional videos consumed with HMD~(Head Mounted Display) headsets. such as the Oculus Rift, Samsung Gear VR and Magic Leap. Users use these devices to enjoy videos shared on social media Facebook and Google YouTube. 
In particular, 360$^{\circ}$~(omnidirectional) videos taken by compact camera devices~(Insta360, Ricoh Theta, and GoPro Max) are becoming immersive in social media platform (Facebook and Google YouTube), because users can use the head-mounted display (HMD) or interactive device to manipulate the viewing direction. 

Because of the numerous applications of omnidirectional images, many approaches have been developed. Single-view depth estimation~\cite{omnidepth,bifuse} predicts depth of the 360$^{\circ}$ scene, considering omnidirectional distortion of the image and convolutional representation~\cite{spherephd}. 
%Depth estimation is a crucial part to interact with the virtual environment. Users can place virtual objects and enjoy the virtual effect. Especially, novel view synthesis~\cite{nerf,nerfw,nerfpp} is essential for immersive augmented and virtual reality. 
Novel view synthesis is a research area that generates image of desired viewpoint by using a learned 3D environment. \jaesik{Cite some papers, and introduce NeRF} View synthesis studies have been developed from MPI~(Multi Plane Images) representation by Zhou~\etal~\cite{stereo_mag}, and NeRF~\cite{nerf} presented neural radiance field representation for synthesis.  %When the user changes the perspective, a novel viewpoint image needs to be generated. For example, networks learn implicit 3D room environments using indoor room video, users could see images of desired viewpoints inside the room and could freely explore the virtual room like the real-world. 

However, the real-world datasets for the 360$^{\circ}$ imaginary are not sufficient compared to the datasets captured by ordinal cameras. Therefore, it is not straightforward to train a neural network model on diverse omnidirectional datasets. 
There exist many datasets titled with \textit{in the wild} captured by the perspective camera from arbitrary environment and camera trajectories~\eg~internet videos so that the learning-based approaches  could be tested with real-world scenes. %Similarly, Robust Vision Challenge 2020\footnote{\url{http://www.robustvision.net/index.php}} tackled the robustness problem that methods trained on indoor dataset often fail to estimate outdoor scenes, and compared state-of-the-art methods on different datasets to evaluate the robustness of the models.
%Not only the diversity of datasets, but also data including moving object~(especially, non-rigid object~\eg~people) could contribute to robustness of models. 
Mannequin Challenge dataset~\cite{frozen_data} was released to solve the problem that the outputs of the depth estimation networks are significantly distracted by the moving objects part in the scene. Specifically, the perspective camera moves around the real-world scene where frozen human, and Structure from Motion~(SfM) and Multi-View Stereo~(MVS) method computes the 3D geometry.
% stands on YouTube videos so that scene depth, including non-rigid object and camera pose are acquired through traditional Structure from Motion~(SfM) and Multi-View Stereo~(MVS) method. 
Thanks to the large number of such videos~\cite{frozen_data}, existing approach could learn depth prediction of dynamic scenes.
%, therefore, computer vision and machine learning community have potential to solves the limitation about geometrical assumption that images of 3D reconstruction are static and not to be contaminated by the moving objects.

In the field of 360$^{\circ}$ datasets, however, most of them are synthetic or a limited amount of real-world scenes captured from a few locations. The deficiency of the 360$^{\circ}$ dataset hinders the extension of the existing approaches, such as depth prediction and view synthesis, to 360$^{\circ}$ images. Therefore, in this study, we introduce a new dataset that consists of 360$^{\circ}$ Youtube videos. Various users and cameras take the videos, and the video shows different places.

Our dataset is the first omnidirectional video data \textit{in the wild} to serve real-world data to the community. 
We propose a pre-processing method to handle raw youtube videos.
%, as most videos are contaminated with many uncertainty factors: editing method containing fade in/out, cut, and transition.
\jaesik{Need to revise}
In particular, we show that the performance of the existing approaches that are trained on monocular depth data and SLAM by obtaining depth and pose by rotating SfM and MVS using a 360-degree dataset. 
Moreover, applying the novel view synthesis network on 360$^{\circ}$ images, the network expandability is shown through the proposed dataset so that the user could explore the implicitly learned 3D space in terms of desired view direction.
\fi

==> tools/README <==

August 26, 2015


The IEEEtrantools.sty package provides several commands from the
IEEEtran.cls file so that they can be used under other LaTeX classes. The
user guide provided here covers only the differences in the use of the
commands from those provided by IEEEtran.cls. For complete documentation
on these commands, see the relevant sections in the IEEEtran_HOWTO manual
of the IEEEtran LaTeX class.

The IEEEtrantools.sty package provides the following IEEEtran.cls commands:

 1. \IEEEPARstart which produces large initial "drop cap" letters.

 2. The \bstctlcite command for the control entry types of IEEEtran.bst
    V1.00 and later.

 3. The \IEEEnoauxwrite command.

 4. The IEEE itemize, enumerate and description list environments.

 5. The complete IEEEeqnarray family for producing multiline equations
    as well as matrices and tables, including the IEEEeqnarray support
    commands.

 6. The \IEEEQEDhere and \IEEEQEDhereams commands to provide amsthm.sty
    \qedhere functionality to IEEEproof. \IEEEQEDhere is for simple use
    "right on the spot" such as within an IEEEeqnarry:

    \begin{IEEEproof}
       \begin{IEEEeqnarray}{rCl+x*}
        x & = & y & \nonumber\IEEEQEDhere
       \end{IEEEeqnarray}
    \end{IEEEproof}

    While \IEEEQEDhereams is like amsthm's venerable \qedhere and is
    for use within the standard equation environment:

    \begin{IEEEproof}
     \begin{equation}
       x = y \nonumber\IEEEQEDhereams\quad
     \end{equation}
    \end{IEEEproof}

    Note that the qedhere style is normally not done with IEEE-related
    work so these are undocumented features of IEEEtran.cls.

    Thanks Mark D. Butala, Hennadiy Leontyev and Stefan M. Moser for
    suggesting this feature.



IEEEtrantools.sty is not needed and should not be used with IEEEtran.cls.

For helpful tips, answers to frequently asked questions and other support,
visit the IEEEtrantools support page at my website:

http://www.michaelshell.org/tex/ieeetran/tools/


Enjoy!

Michael Shell
http://www.michaelshell.org/


*******
2015/08/26 V1.5 (V1.8b of IEEEtran.cls) changes:

 1) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 2) Fix bug with IEEEeqnarray equation number foreground color
    under the color environment of Beamer class.
    Thanks to Joschi Brauchle for reporting this problem.

 3) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.



********************************** Files **********************************

README                - This file.

changelog.txt         - The revision history.

IEEEtrantools.sty     - The LaTeX package file.

IEEEtrantools_doc.txt - The user manual - supplementary to the 
                        IEEEtran_HOWTO manual.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtrantools.sty, IEEEtrantools_doc.txt
***************************************************************************


